Adaptive Height Optimisation for Cellular-Connected UAVs using Reinforcement Learning

Providing reliable connectivity to cellular-connected UAV can be very challenging; their performance highly depends on the nature of the surrounding environment, such as density and heights of the ground BSs. On the other hand, tall buildings might block undesired interference signals from ground BSs, thereby improving the connectivity between the UAVs and their serving BSs. To address the connectivity of UAVs in such environments, this paper proposes a RL algorithm to dynamically optimise the height of a UAV as it moves through the environment, with the goal of increasing the throughput or spectrum efficiency that it experiences. The proposed solution is evaluated in two settings: using a series of generated environments where we vary the number of BS and building densities, and in a scenario using real-world data obtained from an experiment in Dublin, Ireland. Results show that our proposed RL-based solution improves UAVs QoS by 6% to 41%, depending on the scenario. We also conclude that, when flying at heights higher than the buildings, building density variation has no impact on UAV QoS. On the other hand, BS density can negatively impact UAV QoS, with higher numbers of BSs generating more interference and deteriorating UAV performance.

==> biography.tex <==

%\begin{IEEEbiographynophoto}{Luiz A. DaSilva}
%  holds the Telecommunications chair at TCD,
%  where he is the director of CONNECT.
%\end{IEEEbiographynophoto}

%\vfill


==> sections/data-collection.tex <==



==> sections/experiment.tex <==
%\section{Evaluation Description}
%In order to test our algorithm in realistic scenarios we used real-world data from a \ac{uav} flying through Dublin city centre. To complement this evaluation, we investigated the  proposed model in a simulation environment, where we can change the number of BSs and buildings and their distributions. On this section we will explain how the real-world dataset was treated to be used in our analyses, how the simulation was performed and the baselines we use to compare with the proposed solution.
\section{Real-world Data}
\label{sec:experiment-exp}
In order to test our algorithm in realistic scenarios we used real-world data from a \ac{uav} flying through Dublin city centre.
The objective of our proposed algorithm is to maximise \ac{qos} to the UAV at all times, and to evaluate it. We use the data collected in the experimental flights described in \ref{sec:data-exp}, but in order to use the described data we needed to do some cleaning and pre-processing. The evaluation of our proposed height adaptation \ac{DL} model is done with a synthesis of the collected data. In this pre-processing, we do not interfere with any collected values for height, throughput or \ac{SINR}. 

For the synthesis, we have data in the NWQ area from ten different heights, and in the GCQ area nine different heights, each of them separated by 10 meters. As it is separated by 10 m, our increment $d$ is 10. We merge this in a single dataset that simulates that the data was collected at the same horizontal coordinates at the same time. This enables us to know if the \ac{uav} can improve its throughput by changing its height. The goal of our experiment is to use part of this dataset to learn how to select the next movement by predicting which height the \ac{uav} needs to go to in order to achieve a higher \ac{SINR}, then test in the unseen part. 

The data was collected one after another on the same day for each location; however, the time of each flight is slightly different. As the data is collected at different times, meteorological conditions could impact the measured data. 
To be able to use the data, we ignore which time the data was collected. This assumption is needed because we let the \ac{uav} change its height in each time step (steps are 2 seconds); however, on the collected data, there is a considerable difference in time between them.


The horizontal coordinates of each height are also not exactly the same, the UAV was programmed to do the same path, but some factors, such as wind, made it move slightly from height to height. As we assume that the horizontal path only moves straight in the experimental analyses, we needed to make an approximation from the coordinates at each height. Moreover, measurements at certain time steps are missing due to the \ac{uav} not being able to measure as it was performing a handover, jumping 2 seconds on the table. 

For a given flight path, segmented into parts with distinct heights, each segment can vary in the distance travelled. We only consider data points for a given segment where they intersect with the segment with the shortest distance travelled. Otherwise we would not have a complete dataset. We call the flight segment with shortest distance the coordinates base, which for both areas was at 60 m. The coordinate base is the horizontal position we assume the UAV followed during our analysis at every step.
We assumed that the measurements on the other heights were on the coordinate bases precisely coordinates. This means we assume that even if the horizontal coordinates changed slightly for different heights, such as half-meter far from the one at 60 m, we would consider it is the same as in the 60 m. We calculate the distance between the coordinate base and all the coordinates for each height. The smaller calculated distance is considered to be at the same point as the coordinate base. With this procedure, the \ac{uav} has the closest coordinates for all heights, and we can assume its path is approximately a straight line. 

Each set of measurements at given coordinates corresponds to a single discrete step in our evaluation. The starting position $z_1$ is fixed, and afterwards, it is controlled by the action selection process of our proposed \ac{dql} algorithm described in Section~\ref{sec:ml} or by the baseline solution algorithm. Table \ref{table:sample-data-uav-changed} illustrates an sample of the data after the pre-processing. The data does not have information of the time. The coordinates are aligned, the step is defined for each line, and it is defined that height of each measurement.


\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\rowcolor[HTML]{C0C0C0} 
Step & Height &  Latitude & Longitude & SINR Carrier 1 (dB)  & Serving Cell Identity &  Throughput (kbps)\\ \hline
1 & 20 & 53.34342193604 & -6.23032475884304 & 10.3
 &  60 & 46761.22  \\ \hline
1 & 30 & 53.34342193604 & -6.23032475884304 & 20.2 &  60 & 76651.78  \\ \hline
1 & 40 & 53.34342193604  & -6.23032475884304 & 11.1
&  60 & 46797.87 \\ \hline 
1 & 50 & 53.34342193604 & -6.23032475884304 & 6.4
 &  61 &  35082.27\\ \hline 
1 & 60 & 53.34342193604 & -6.23032475884304 & 3.4
&  61 & 29024.27 \\ \hline 
1 & 70 & 53.34342193604 & -6.23032475884304 & 9.9
& 60 & 46738.80 \\ \hline 
\end{tabular}
}
\caption{
Sample of data from GCQ area after pre-processing to be used in the evaluation.
	}
	\label{table:sample-data-uav-changed}
\end{table}


The hyper-parameters that provided the best results are illustrated in Table \ref{table:rl-exp}. However, we needed to perform a deep investigation to choose the hyper-parameters and design the model. 
We changed several of the hyper-parameters and inputs of the model until finding the proposed one.
These parameters were experimentally selected among a number of model variations in which the number of layers, number of neurons per layer, activation function, number of epochs, regularisation, and the inputs were varied.  As we apply experience replay, the epochs are how many times the model is trained with the mini-batch at each time-step. 
Depending on the complexity of the \ac{dql} network (for example number of input features, number and size of layers), the training can be performed in a few steps, or require thousands or larger number of steps. However, for the \ac{uav} height adaptation scenario it is imperative to have as few training steps as possible, so that the model can learn to optimise height quickly in any new city environment is applied in. %The value of epsilon decay in our evaluation is small compared to other \ac{dql} applications, which makes it learn quickly. %; it is because our model is trained in each new environment.
In order to have a fast adaptation in a new environment, the model needs to adapt its weights quickly to not interfere with the UAV performance at the end of the path. For this evaluation, the value of $\epsilon$ and $\epsilon$-decay are 1 and 0.9 respectively, effectively meaning that the proposed model trains in 30 steps. We apply replay memory as an strategy to accelerate the learning process, where at each step the model trains with the mini batch for the number of epochs.

\begin{table}[t]
\centering
\begin{tabular}{|c|c|}
\hline
\rowcolor[HTML]{C0C0C0} 
Parameters & Value \\ \hline
Epoch & 200 \\ \hline
Epsilon & 1 \\ \hline
Epsilon\_decay & 0.9 \\ \hline
Neurons per hidden layer & 200 \\ \hline
Number of hidden layers & 3 \\ \hline
Regularisation after hidden layers & RELU \\ \hline
Output layer & Softplus \\ \hline
Optimisation function & Adam \\ \hline
\end{tabular}
\caption{
Values of hyper-parameters for the proposed DQN model used in evaluation.
	}
	\label{table:rl-exp}
\end{table}

\subsection{Simulation}
\label{sec:experiment-sim}

\begin{table}[t]
\centering
\begin{tabular}{|c|c|}
\hline
\rowcolor[HTML]{C0C0C0} 
Variable & Value \\ \hline
$Z_{min}$ &  40 $m$ \\ \hline
$Z_{max}$ &  240 $m$ \\ \hline
$BS_{dens}$ & $[1,2.5,5] /km^2$ \\ \hline
Bs height $z_{b}$ &  $30 m$ \\ \hline
BS downtilt $\phi$ & 30 \\ \hline
$Build_{dens}$ & $[1,2,3]*100 /km^2$ \\
\hline
Building area  $Bl_a$ & 40 $m^2$ \\ \hline
Building height parameter a & 20 $m$ \\ \hline
Simulated area & 3 $km^2$ \\ \hline
Horizontal Speed & 10 $m/s$ \\ \hline 
Timestep & 1 $s$ \\ \hline 
Distance between $x_i$ and $x_f$   & 1000 $m$ \\ \hline 
Step & 100 \\ \hline 
d & 10 m \\ \hline 
Mctrials & 100 \\ \hline 
\end{tabular}
\caption{
Simulation parameters.
	}
	\label{table:simu}
\end{table}

To evaluate our proposed approach and analyse how the city topology influences the connected \ac{uav}, we utilise the simulator developed in R \cite{boris_dic_ant}. 
In this experiment we want to vary the building and \ac{bs} densities in order to evaluate the generalisation of our model.

%A Mctrial, or Marco Carlos simulation, is a model used to predict the probability of different outcomes once the simulation environment changes its characteristics randomly. 
For the experiment analyses, we have the equivalent of 2 Mctrial, and we test the model on that environment 100 times, starting the model from scratch at each time, so it does not overfit. In order to evaluate the model in different environments, for each MCtrial, we randomly generate the \ac{bs} and buildings distribution, so the \ac{uav} always observes a "new environment" at every 100 steps.
During the each run, we do not vary the \ac{bs} and the building densities at the same time, always letting one of the variables to remain fixed so we can evaluate the impact of each. The chosen value to be the fixed is the mean of the list values, and shown in Table \ref{table:simu} with other simulation parameters.
A step (or timestep) is a single movement (action taken) of the \ac{uav} in a specific \ac{bs} and building topology. We assumed the minimum allowed height $Z_{min}$ as 40 m, because of simplification for the simulation, as with the \ac{uav} achieving the minimum of 40 m it would above the buildings. We wanted to investigate if a increase of the maximum height $Z_{max}$ allowed for the \ac{uav} to fly could be beneficial to its \ac{qos}, then we increased from 120 m in Chapter \ref{chap:height-experiment} to 240 m in the simulation. The \ac{bs} density $BS_{dens}$, \ac{bs} height $z_{b}$, building area $Bl_a$, building density $Build_{dens}$ and building height are based on the ITU specification  \cite{series2013propagation}.


\subsection{Baselines}
\label{sec:baseline}
We choose five different height selection strategies to which we compare performance of our proposed \ac{rl} algorithm. 
For the first one, we use the baseline proposed by Zhang \cite{trajec-mobile}, which suggests that the \ac{uav} maintain the minimum allowed height during its flight. One of the most common approaches to \ac{uav} height selection is to maintain a constant height \cite{nallanathan,rami1,reshape,network-adapt}, but there is no consensus on which height value to choose. To make a fair comparison, we also benchmark our approach against two constant height values. These heights will be the maximum possible height, and half of the maximum. When following these fixed height strategies, the \ac{uav} will begin at the minimum height at timestep 1, before increasing its height in each timestep until it reaches the required height, after which it will make no further adjustments.

To confirm that our solution is actually learning based on observed environment information and not acting randomly, we also compare it to a bounded Random walk height selection strategy, in which the \ac{uav} in each timestep randomly selects one of  three actions: increase the height, decrease the height, or keep the current height. It is bounded as all the solutions and cannot fly outside the allowed flight range. 

In order to compare our solution to a more complex baseline, we implement an approach that we call One-step-ahead solution. In the One-step-ahead approach, the \ac{uav} knows whether the maximum \ac{SINR} in the next time step will be found above or below its current height, and will move up or down (in a fixed increment of d = 10 m) depending on this knowledge. To be able to apply the One-step-ahead solution, the \ac{uav} needs previous information about  the environment; this is not feasible in a real-world application, but we include this to assess whether and by how much  such information would improve performance when compared to our \ac{rl} approach.

We also compare our \ac{rl} solution with  one based on optimal height at each time step as obtained from the real-world dataset. In this approach, it is assumed that the \ac{uav} is able to move to any height in the next timestep, without restrictions of $d$. This represents the ideal-case performance which would not be possible in a real-world \ac{uav} application.

Bellow are benchmark approaches:
\begin{itemize}
    \item \textbf{Zhang \cite{trajec-mobile}}: this benchmark proposes that the \ac{uav} should maintain the minimal allowed height at all times.
    \item \textbf{Constant at  60 m}: this benchmark starts at the minimal height, like all others, and then moves up at every step until it achieves 60 m height. After achieving 60 m, the \ac{uav} should not move up or down.
    \item \textbf{Constant at  120 m}: this benchmark starts at the minimal height, like all others, and then moves up at every step until it achieves 120 m height. After achieving 120 m, the \ac{uav} should not move up or down.
    \item \textbf{Random walk}: this benchmark chooses its action randomly at each step.
    \item \textbf{Optimal height}: this is a reference benchmark of the maximum possible \ac{qos} values. In this approach, the \ac{uav} does not have any limitations on the maximum height change from step to step and also know which height has the maximum \ac{qos}. 
    \item \textbf{One-step-ahead}: this benchmark follows the optimal height next position to decide its next action. If in the next step the optimal height is above the actual height of the \ac{uav}, the chosen action will be to move up. If in the next step the optimal height is bellow the actual height of the \ac{uav}, the chosen action will be to move down. In case the optimal height in the next step is the same as the actual height, the \ac{uav} should not move.
\end{itemize}


